A Multistep Frank-Wolfe Method

The Frank-Wolfe algorithm has regained much interest in its use in structurally constrained machine learning applications. However, one major limitation of the Frank-Wolfe algorithm is the slow local convergence property due to the zig-zagging behavior. We observe the zig-zagging phenomenon in the Frank-Wolfe method as an artifact of discretization, and propose multistep Frank-Wolfe variants where the truncation errors decay as $O(\Delta^p)$, where $p$ is the method's order. This strategy "stabilizes" the method, and allows tools like line search and momentum to have more benefits. However, our results suggest that the worst case convergence rate of Runge-Kutta-type discretization schemes cannot improve upon that of the vanilla Frank-Wolfe method for a rate depending on $k$. Still, we believe that this analysis adds to the growing knowledge of flow analysis for optimization methods, and is a cautionary tale on the ultimate usefulness of multistep methods.

==> sections/checklist.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  
 For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}

Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/discussion.tex <==
\section{Discussion}
The goal of this work is to put forth a thorough analysis of multistep methods over the flow system captured by the Frank-Wolfe method. Our results are numerically promising but theoretically disheartening; on the one hand, because the flow system does not zig-zag, better discretization methods do offer more stable search directions and momentum performance. On the other hand, because truncation error ultimately dominates convergence error, better multistep methods in general cannot improve local convergence rates. This   discovery  has implications not just for Frank-Wolfe methods, but for \emph{any} multistep optimization methods to beat the original convergence rates, and is a cautionary tale for assuming too much from a beautiful flow rate.

%From the analysis and numerical results, we believe we have put forth a convincing argument that reducing zig-zagging by reducing discretization error indeed improves the performance of Frank-Wolfe methods, simply by suppressing zig-zagging behavior. However, our negative result shows that there is no hope of achieving a better \emph{convergence rate}. Additionally, we
%offer intuition to say that better discretization methods in general may not be a key to better optimization methods, as discretization error always dominates local convergence error in the long run. 

%Therefore it is imperative to somehow exploit the quality of ``better step direction", offered by eliminating zig-zagging. Here, we offer two solutions: better line search, and better acceleration from momentum-based methods; however, we believe this area is still open for more improvements.

==> sections/frankwolfe.tex <==
\section{The Frank-Wolfe method}
The \FW~methodhas become popular in structural optimization, when in particular one desires a solution $\bx^*$ that is a sparse convex combination of a special class of vectors (often called \emph{atoms}). These atoms then form the vertices of $\mD$, and the operation $\lmo$ extracts the vertex that is most correlated with the steepest descent direction at each iteration. 
This vertex $\bs^{(k)}$ is then mixed into the iterate $\bx^{(k)}$ with mixing coefficient $\gamma^{(k)}$, whose decay rate plays an important role in the convergence rate of \FW. 

%\paragraph{Sparse optimization.}
%For example, in sparse element-wise optimization, the constraint $\bx\in \mD$ is often manifested as a limit on the sparse norm of $\bx$, e.g. $\|\bx\|_1\leq \alpha$ for some hyperparameter $\alpha \geq 0$. The LMO in this case is simply
%\[
%\lmo_\mD(\bx) = -\alpha\, \sign((\nabla f(\bx))_j)\,\be_j,\qquad
%j = \argmax{i}\, |(\nabla f(\bx))_j|
%\]
%where $\be_k$ is a standard basis vector (one-hot at position $k$). 
%Notice that the complexity of this LMO operation is simply that of finding the index of the largest element in a vector,  $O(n)$. In contrast, a projection on the one-norm ball is considerably more involved. 


%\paragraph{Low-rank optimization.} The low complexity benefit of LMOs is even starker in the case of low-rank optimization, often modeled by forcing $\|X\|_*\leq \alpha$, where $\|X\|_*$ is the nuclear norm (maximum singular value) of a matrix variable $X$.  Here, both the projection on the level set \emph{and} the proximal operator of the nuclear norm requires full spectral calculations. In contrast, the LMO only requires knowing the eigenspace associated with the \emph{largest} singular value, an operation often achieved much more efficiently. 

%\paragraph{The tradeoff}
While the per-iteration complexity of FW can be appealing, the downside is that the convergence rate is usually slow, compared against projected gradient methods \citep{jaggi2013revisiting,lacoste2015global,freund2016new}; in particular, without special assumptions beyond smoothness, away steps, or use of line search, the best known convergence rate of  \FW~is $O(1/k)$. 
%In fact, we will later show that, for a generalized class of step sizes, this is the best possible rate.

%\begin{proposition}\label{prop:fwlowerbound}
%Suppose that $\gamma_k = \frac{c}{c+k}$, for some constant $c\geq 1$. Then, for any choice of $c$, the method \FW~has a lower bound of $f(\bx^{(k)})-f^* = \Omega(1/k)$.
%\end{proposition}
%The proof is given in the appendix, but can be seen simply by tracking the rate of decay of the iterates over the 1-D problem
%\[
%\minimize{-1\leq x\leq 1} \; \tfrac{1}{2} x^2
%\]
%with any $\bx^{(0)} \neq 0$.
%\red{Revisit this. should we not just say it's a consequence of RK?}
%Note that in this example problem, the vanilla FW method oscillates between $\bs^{(k)} = 1$ and $\bs^{(k)} = -1$ at every step.

%However, the same fundamental bad rate  disappears in the continuous time limit.

%In this paper, we explore this fundamental rate as it applies to the continuous \FWflow~and its various discretizations.





==> sections/proofs.tex <==


\begin{lemma}
Consider the iterative sequence
\[
x^{(k+1)} = x^{(k)}-\gamma^{(k)} (x^{(k)}+\sign(x^{(k)})
\]
and assume that for some $\bar k$, 
\[
|x^{(\bar k)}| < \frac{\gamma^{(\bar k)}}{1-\gamma^{(\bar k)}}.
\]
Then for all $k\geq \bar k$, $\sign(x^{(k)}) \neq \sign(x^{(k+1)})$.
\end{lemma}

At each iteration, 
\[
|x^{(k+1)}| = 
\begin{cases}
(1-\gamma^{(k)})|x^{(k)}| - \gamma^{(k)}
& \text{ if } \sign(x^{(k)})= \sign(x^{(k+1)})
\\
\gamma^{(k)} - (1-\gamma^{(k)})|x^{(k)}| & \text{ if } \sign(x^{(k)})\neq \sign(x^{(k+1)})
\end{cases}
\]

That is, 
\[
\sign(x^{(k)})\neq \sign(x^{(k+1)})
\iff
\gamma^{(k)} > (1-\gamma^{(k)})|x^{(k)}|
\]
Furthermore, assuming the previous point oscillated,
\begin{eqnarray*}
\sign(x^{(k+1)})\neq \sign(x^{(k+2)})
\iff
\gamma^{(k+1)} &>& (1-\gamma^{(k+1)})\red{(\gamma^{(k)}-(1-\gamma^{(k)})|x^{(k)}|)}\\
\sign(x^{(k+2)})\neq \sign(x^{(k+3)})
\iff
\gamma^{(k+2)} &>& (1-\gamma^{(k+2)})\blue{(\gamma^{(k+1)}-(1-\gamma^{(k+1)})}\red{(\gamma^{(k)}-(1-\gamma^{(k)})|x^{(k)}|)}\blue{)}\\
\sign(x^{(k+3)})\neq \sign(x^{(k+4)})
\iff
\gamma^{(k+3)} &>&
(1-\gamma^{(k+3)})(\gamma^{(k+2)}-(1-\gamma^{(k+2)})\blue{(\gamma^{(k+1)}-(1-\gamma^{(k+1)})}\red{(\gamma^{(k)}-(1-\gamma^{(k)})|x^{(k)}|)}\blue{)})\\
\end{eqnarray*}

Does
\[
\gamma^{(k)} > (1-\gamma^{(k)})|x^{(k)}|
\]
imply 
\[
\gamma^{(k+2)} > (1-\gamma^{(k+2)})\blue{(\gamma^{(k+1)}-(1-\gamma^{(k+1)})}\red{(\gamma^{(k)}-(1-\gamma^{(k)})|x^{(k)}|)}\blue{)}?
\]

Define
\[
\rho = \gamma^{(k)} - (1-\gamma^{(k)})|x^{(k)}|, 
\]
and assume $\rho > 0$. Then

\[
\frac{\gamma^{(k+2)}}{(1-\gamma^{(k+2)})} = \frac{c}{k+2} %\overset{?}
{>} \blue{(\frac{c}{c+k+1}-\frac{k+1}{c+k+1}}\red{\rho}\blue{)}?
\]
which is true if $c \geq 1$.

More broadly, this is true if 
\[
\frac{\gamma^{(k+2)}}{(1-\gamma^{(k+2)}} \geq \gamma^{(k+1)}
\]



Does
\[
\gamma^{(k+1)} > (1-\gamma^{(k+1)})\red{(\gamma^{(k)}-(1-\gamma^{(k)})|x^{(k)}|)}
\]
imply
\[
\gamma^{(k+3)} > (1-\gamma^{(k+3)})(\gamma^{(k+2)}-(1-\gamma^{(k+2)})\blue{(\gamma^{(k+1)}-(1-\gamma^{(k+1)})}\red{(\gamma^{(k)}-(1-\gamma^{(k)})|x^{(k)}|)}\blue{)})?
\]
Define
\[
\mu = \gamma^{(k+1)} - (1-\gamma^{(k+1)})\red{(\gamma^{(k)}-(1-\gamma^{(k)})|x^{(k)}|)} > 0
\]
Require
\[
\frac{\gamma^{(k+3)}}{(1-\gamma^{(k+3)})} > (\gamma^{(k+2)}-(1-\gamma^{(k+2)})\mu)?
\]
which is true if 
\[
\frac{\gamma^{(k+3)}}{(1-\gamma^{(k+3)})} \geq \gamma^{(k+2)}
\]
and plugging in $\gamma^{(k)} = \frac{c}{c+k}$
\[
\frac{c}{k+3} \geq \frac{c}{c+k+2}
\]
which is true for $c\geq 1$.

So, if there exists a $\bar k$ where 
\[
\gamma^{(\bar k)} > (1-\gamma^{(\bar k)})|x^{(\bar k)}|, \qquad
\gamma^{(\bar k+1)} > (1-\gamma^{(\bar k+1)})\red{(\gamma^{(\bar k)}-(1-\gamma^{(\bar k)})|x^{(\bar k)}|)}
\]



then for all future $k\geq \bar k$, $\sign(x^{(k+1)})\neq \sign(x^{(k)})$.

The conditions $(\star)$ for $\bar k = k$ is equivalent to 
\[
\frac{\gamma^{(k)}}{(1-\gamma^{(k)})}> |x^{(k)}| > \left(\gamma^{(k)}-\frac{\gamma^{(k+1)}}{1-\gamma^{(k+1)}}\right)\cdot \frac{1}{(1-\gamma^{(k)})}
\]

plug in $\gamma^{(k)}=\frac{c}{c+k}$

\[
\frac{c}{k} > |x^{(k)}| > \left(\frac{c}{c+k}-\frac{c}{k+1}\right)\cdot \frac{c+k}{c}
 = \frac{1-c}{k+1}
\]
The second inequality is trivally true since the right hand side is negative. (More generally, this is trivially true if 
$\gamma^{(k)} < \frac{\gamma^{(k+1)}}{1-\gamma^{(k+1)}}$.)

\section{New proofs}


\begin{lemma} 
After one step, the generalized Runge-Kutta method satisfies
\[
h(x_{k+1})-h(x_k) \leq
\]
where $h(x) = f(x) - f(x^*)$.
\label{lem:rungekutta-positive-onestep}
\end{lemma}
\begin{proof}
For ease of notation, we write $x = x_k$ and $x^+ = x_{k+1}$.
Now consider the generalized RK method
\begin{eqnarray*}
\bar x_i &=& x + \sum_{j=1}^p A_{ij} \xi_j\\
\xi_i &=& \underbrace{\frac{c}{c+k+\omega_i}}_{\tilde \gamma_i} \underbrace{\left( s_i - \bar x_i \right)}_{\tilde x_i}\\
x^+&=&  x + \sum_{i=1}^p \beta_i \xi_i\\
\end{eqnarray*}
where $s_i = \lmo(\bar x_i)$.


Since $x\in \mD$ and $s_i\in \mD$ for all $i$, then recursively, (starting with $\bar x_1 = x\in \mD$)
\begin{eqnarray*}
\bar x_2 &=& x + \tilde \gamma_1 A_{2,1}(s_1- x)\\
&=& \left(1-\tilde \gamma_1 A_{2,1}\right) x + \tilde \gamma_1 A_{2,1} s_1\in \mD\\
\bar x_3 &=& x + \tilde \gamma_1 A_{3,1}(s_1- x) + \tilde \gamma_2 A_{2,1}(s_2- \bar x_2)\\
&=& \alpha \bar x_2 + (1-\alpha) x + \underbrace{\tilde \gamma_1 (A_{3,1}- \alpha A_{2,1})}_{\alpha}(s_1- x) + \underbrace{\tilde \gamma_2 A_{2,1}}_{\leq 1-\alpha}(s_2- \bar x_2) \in \mD\\
\end{eqnarray*}
and so forth, and \red{as long as conditions are met for $\alpha$ to exist}, $\bar x_i\in \mD$.

Now, we establish some bounds. Define $D = \diam(\mD)$. Then for all $x,y\in D$, $\|x-y\|_2\leq D$. Therefore, 
\[
\|x-\bar x_i\|_2 = \|\sum_{j=1}^p A_{ij}\xi_j\|_2 \leq p\max_{ij}|A_{ij}| \frac{c}{c+k} \|s_i-\bar x_i\|_2\leq \underbrace{Dp\max_{i,j}|A_{ij}|}_{=:D_2}\underbrace{\frac{c}{c+k}}_{=\gamma}
\]
and similarly, $\|s-\bar x_i\|_2\leq D_2\gamma$.

Then 
\begin{eqnarray*}
f(x^+)-f(x) &\leq&  \nabla f(x)^T(x^+-x) + \frac{L}{2}\|x^+-x\|_2^2\\
&=&  \sum_i \beta_i \tilde \gamma_i \nabla f(x)^T(s_i-\bar x_i) + \frac{L}{2}\underbrace{\|\sum_i \beta_i \tilde \gamma_i (s_i-\bar x_i)\|_2^2}_{\leq \gamma^2 D_2^2}\\
&=&  \sum_i \beta_i \tilde \gamma_i (\nabla f(x)-\nabla f(\bar x_i))^T(s_i-\bar x_i) +
 \sum_i \beta_i \tilde \gamma_i \underbrace{\nabla f(\bar x_i)^T(s_i-\bar x_i)}_{\gap(\bar x_i)} +
 \frac{L\gamma^2D_2^2}{2}\\
 &\leq& \sum_i \beta_i\underbrace{ \tilde \gamma_i}_{\leq \gamma} \underbrace{\|\nabla f(x)-\nabla f(\bar x_i)\|_2}_{L\|x-\bar x_i\|_2=L\gamma D_2}\underbrace{\|s_i-\bar x_i\|_2}_{\leq D_2} - \sum_i \beta_i\tilde\gamma_i \gap(\bar x_i) + \frac{L\gamma^2 D_2^2}{2}\\
 &\leq &  -\sum_i \beta_i\tilde\gamma_i \gap(\bar x_i) + \frac{3L\gamma^2 D_2^2}{2}\\
 &\leq& -\gamma^+ \sum_i\beta_i h(\bar x_i) + \frac{3L\gamma^2 D_2^2}{2}
\end{eqnarray*}
where $h(x) = f(x) -f(x^*)$, $\gamma=\gamma_k$, and $\gamma^+=\gamma_{k+1}$. Now assume $f$ is also $L_2$-continuous, e.g. $|f(x_1)-f(x_2)|\leq L_2\|x_1-x_2\|_2$. Then

\begin{eqnarray*}
h(x^+)-h(x) 
 &\leq& -\gamma^+ \sum_i\beta_i (h(\bar x_i)-h(x)) -\gamma^+ \underbrace{\sum_i\beta_i}_{=1} h(x) + \frac{L\gamma^2 D_2^2}{2}\\
 &\leq & \underbrace{\gamma \sum_i\beta_iL_2 \|\bar x_i-x\|_2}_{\propto\gamma^2}-\gamma^+ h(x) + \frac{L\gamma^2D_2^2}{2}\\
 &\leq& -\gamma^+ h(x) + D_3(\gamma^+)^2
\end{eqnarray*}
where $D_3 =2( D_2^2 + 3\frac{LD_2^2}{2})$ and we use $2 \geq (\gamma/\gamma^+)^2$ for all $k \geq 1$.

\end{proof}


\begin{proposition} 
The generalized Runge-Kutta method converges with $O(1/k)$ rate.
\label{prop:rungekutta-positive}
\end{proposition}

\begin{proof}
After establishing Lemma \ref{lem:rungekutta-positive-onestep}, the rest of the proof is a recursive argument, almost identical to that in \cite{jaggi2013revisiting}. 

At $k = 0$, we define $h_0 =\max\{ h(x_0), \frac{ D_3c^2}{c-1}\}$, and it is clear that $h(x_0) \leq \frac{h_0}{k+1} = h_0$.

Now suppose that for some $k$, $h(x_k) \leq \frac{h_0}{k+1}$. Then
\begin{eqnarray*}
h(x_{k+1}) &\leq &  h(x_k) - \gamma_{k+1}h(x_k) + D_3 \gamma_{k+1}^2\\
&=& \frac{h_0}{k+1}\cdot \frac{k+1}{c+k+1} + D_3 \frac{c^2}{(c+k+1)^2}\\
&=& \frac{h_0}{c+k+1} + D_3 \frac{c^2}{(c+k+1)^2}\\
&=& \left( h_0 + \frac{D_3c^2}{c+k+1}\right) \left(\frac{k+2}{c+k+1}\right) \frac{1}{k+2}
\\
&\leq& h_0\left( 1+\frac{c-1}{c+k+1}\right) \left(\frac{k+2}{c+k+1}\right) \frac{1}{k+2}\\
\\
&\leq& h_0\underbrace{\left( \frac{2c+ k }{c+k+1}\right) \left(\frac{k+2}{c+k+1}\right)}_{\leq 1} \frac{1}{k+2}.
\end{eqnarray*}

\end{proof}


\begin{assumption}\label{asspt:betacancel}
The choice of $\beta\in \R^p$ is not ``cancellable"; that is, there exist no partition $S_1\cup S_2 =\{1,...,p\}$ where 
\[
\sum_{i\in S_1}\beta_i - \sum_{j\in S_2} \beta_j = 0.
\]
\end{assumption}
This is true for most of the higher order  Runge-Kutta methods. However, even in cases where  Assumption \ref{asspt:betacancel} does not hold, our numerical experiments have never shown this assumption to be necessary; it is merely there to aid the proof. (Translation: do not design your Runge Kutta method for the $\beta$'s to be cancel-able in hopes of achieving a better rate!)



\begin{proposition} Start with $x_0 = 1$. Then regardless of the order $p$ and choice of $A$, $\beta$, and $\omega$, as long as $\sum_i \beta_i = 1$ and assumption \ref{asspt:betacancel} holds, then 
\[
\sup_{k'>k} |x_k| =\Omega(1/k).
\]
That is, the tightest upper bound is $O(1/k)$.
\label{prop:rungekutta-negative}
\end{proposition}


\begin{lemma}[$O(1/k)$ rate]
Start with $x_0 = 1$. Then consider the sequence defined by
\[
x_{k+1}= |x_k - \frac{c_k}{k}|
\]
where, no matter how large $k$ is, there exist some constant where  $C_1 < \max_{k'>k} c_{k'} $.
(That is, although $c_k$ can be anything, the smallest upper bound of $c_k$ does not decay.) Then
\[
\sup_{k'\geq k} |x_{k'}| = \Omega(1/k).
\]
That is, the smallest upper bound of $|x_k|$ at least of order $1/k$.
\end{lemma}
\begin{proof}
We will show that the smallest upper bound of $|x_k|$ is larger than $\epsilon/(2k)$.


Proof by contradiction. 
Suppose that at some point $K$, for all $k \geq K$,  $|x_{k}| < \epsilon/(2k)$. Then from that point forward, 
\[
\sign(x_k-\frac{c_k}{k}) = -\sign(x_k)
\]
and there exists some $k' > k$ where $c_{k'} > C_1$. Therefore, at that point,
\[
|x_{k'+1}| = \frac{c_{k'}}{k'}-|x_{k'}| 
\geq \frac{C_1}{2k'}>\frac{C_1}{2(k'+1)}.
\]
This immediately establishes a contradiction.
\end{proof}



Now define the Runge Kutta operator
\[
T(x) = \sum_{i=1}^p \beta_i \xi_i,
\]
and note that 
\[
|x_{k+1}| = |x_k+T(x_k)| = | |x_k|+\sign(x_k)T(x_k)|.
\]
Thus, if we can show that there exist some $\epsilon$, agnostic to $k$ (but possibly related to Runge Kutta design parameters), and
\begin{equation}
\exists k'\geq k, \quad -\sign(x_{k'})T(x_{k'}) > \frac{\epsilon}{k'},\quad \forall k,
\label{eq:lemma-helper-1}
\end{equation}
 then based on the previous lemma, this shows $\sup_{k'>k}|x_{k'}| = \Omega (1/k)$ as the smallest possible upper bound.



\begin{lemma}
There exists a finite point $\tilde k$ where for all $k > \tilde k$, $\|\xi\|_\infty < O(1/k)$.
\end{lemma}
\begin{proof}
Assume first that $\tilde k > -\min_i \omega_i$; thus $k+\omega_i > 0$ for all $k > \tilde k$. Next,
suppose that at some point, $\|\xi\|_\infty < C$ for some constant $C>0$. Then 
\[
|\xi_i| = \frac{c}{c+k+\omega_i} \left| x_k+  \sum_{j=1}^p A_{ij} \xi_j + q_i\right|\leq 
\frac{c}{c+k+\min_j\omega_j} \left| 2+  p\max_{i,j}|A_{ij}| \right| < C
\]
if
\[
k>\frac{c}{C} \left( 1+  p\max_{i,j}|A_{ij}| + 1-C\right)-\min_j\omega_j 
\]
which is satisfied if 
\[
k>c(2+p\max_{i,j}|A_{ij}|).
\]
That is, from that point forward, $\|\xi\|_\infty$ is a decaying sequence in $t$.

Now that we have established that, when $k$ is large enough, there exist some $C$ where $\|\xi\|_\infty < C$ for all $k'>k$, then it also must be that 
\[
|x_k+\sum_jA_{ij}\xi_j+q_i| <2+p\max_{ij}|A_{ij}|C<C_2
\]
and thus for future $k$,
\[
|\xi_i| < \frac{C_2 c}{c+k+\omega_i}<\frac{C_2 c}{c+k}
\]
and therefore 
\[
\|\xi\|_\infty<\frac{C_2 c}{c+k}.
\]
\end{proof}


\begin{lemma}
There exists a finite point $\tilde k$ where for all $k > \tilde k$, 
\[
 \frac{c}{c+k}-\frac{C_2}{k^2} < |\xi_i| < \frac{c}{c+k}+\frac{C_2}{k^2}
\]
for some constant $C_2>0$.
\end{lemma}
\begin{proof}
From \red{the previous lemma} we have that
\[
|x_k+\sum_j A_{ij}\xi_j|<\frac{C_3}{k}
\]
for some $C_3>0$.
Then
\[
1-\frac{C_3}{k}\leq 1-x_k+\sum_j A_{ij}\xi_j\leq |x_k+\sum_j A_{ij}\xi_j+q_i| \leq 1+x_k+\sum_j A_{ij}\xi_j\leq 1+\frac{C_3}{k}.
\]
Therefore
\[
\frac{c}{c+k+\omega_i}(1-\frac{C_3}{k}) \leq |\xi_i| \leq  \frac{c}{c+k+\omega_i}(1+\frac{C_3}{k}).
\]
The upper bound simplifies as
\[
\frac{c}{c+k+\omega_i}(1+\frac{C_3}{k})\leq \frac{c}{c+k}(1+\frac{C_3}{k})\leq \frac{c}{c+k}+\frac{C_3}{k^2}.
\]
We can further clean up the lower bound as
\[
 \frac{c}{c+k+\omega_i}= \frac{c}{c+k}-\frac{c\omega_i}{(c+k)(c+k-\omega_i)}
 \]
so
\[
\frac{c}{c+k}-\frac{c\omega_i}{(c+k)(c+k-\omega_i)}\leq |\xi_i| \leq   \frac{c}{c+k}+\frac{C_3c}{k(c+k)}
\]
Pick $k >2\omega_{\max}$. Then
\[
\frac{c\omega_i}{(c+k)(c+k-\omega_i)}\leq \frac{2c\omega_{\min}}{(c+k)(2c+k)}\leq \frac{2c\omega_{\min}}{k^2}.
\]
Therefore, using $\tilde k > 2\max_i \omega_i$ and $C_2 > \max\{C_3,2c\omega_{\min}\}$ completes the proof.
\end{proof}






\begin{lemma}
There exists some large enough $\tilde k$ where for all $k \geq \tilde k$, it must be that
\begin{equation}
\exists k'\geq k, \quad -\sign(x_{k'})T(x_{k'}) > \frac{\epsilon}{k'}.
\label{eq:lemma-helper-1}
\end{equation}
\end{lemma}

\begin{proof}
Define a partitioning $S_1\cup S_2 = \{1,...,p\}$, where
\[
S_1 = \{i : \xi_i > 0\}, \quad S_2 = \{j : \xi_j\leq 0\}d.
\]
Defining $\bar \xi = \frac{c}{c+k}$,
\[
|\sum_{i=1}^p \beta_i \xi_i| = |\sum_{i\in S_1}\beta_i |\xi_i| -\sum_{j\in S_2}\beta_j|\xi_j|| \geq  \left(\bar \xi-\frac{C_2}{k^2}\right)\cdot\left|\sum_{i\in S_1}\beta_i-\sum_{j\in S_2}\beta_j\right|.
\]

Assumption \ref{asspt:betacancel} says that there does not exist a combination of $\beta_i$ where a specific linear combination could cancel them out; that is, suppose that there exists some constant $\bar \beta$, where for \emph{every} partition of sets $S_1$,$S_2$,
\[
0<\bar\beta :=\min_{S_1,S_2}  |\sum_{i\in S_1}\beta_i-\sum_{j\in S_2}\beta_j|.
\]
Then  
\[
|\sum_{i=1}^p \beta_i \xi_i|  \geq  \left(\frac{c}{c+k}-\frac{C_2}{k^2}\right)\bar\beta \geq \frac{\bar\beta}{2}\frac{c}{c+2}
\]
when 
\[
k>\frac{C_2}{c} \Rightarrow \frac{C_2}{k^2}<\frac{c/2}{c+k}.
\]
This concludes the proof.
\end{proof}




























\iffalse
\begin{lemma}
Consider the problem 
\[
\minimize{x}\quad \left\{\frac{1}{p} x^p : -1\leq x \leq 1\right\}
\]
where $p$ is even and positive. Assume that for all $\gamma^{(k)}$,
\[
\frac{\gamma^{(k+1)}}{1-\gamma^{(k+1)}} \geq \gamma^{(k)},\qquad \forall k.
\]
Then Frank-Wolfe will always oscillate for $k$ large enough.
\end{lemma}

\begin{proof}
At each iteration, 
\[
x^{(k+1)} = x^{(k)} - \gamma^{(k)}(x^{(k)}+\sign(x^{(k)})).
\]
So, all we have to do is show that no matter what $x^{(0)}$ is, as long as $-1\leq x^{(0)} \leq 1$, then there exists a $\bar k$ where $|x^{(\bar k)}|\leq \frac{\gamma^{(k)}}{1-\gamma^{(k)}}$.

Define $\theta^{(k)} = \frac{(1-\gamma^{(k)})}{\gamma^{(k)}}$. Then we wish to show that for some $\bar k$, 
\[
\theta^{(\bar k)}|x^{(\bar k)}|\leq 1.
\]

Notice that if \[
\theta^{(\bar k)}|x^{(\bar k)}|\leq 1 \iff \sign(x^{(k)}) \neq \sign(x^{(k+1)})
\]
which also means that any point, if the sign changes, then all future signs will change. 



So, now assume that for all $k$, $\sign(x^{(k)})=\sign(x^{(k+1)}$, or that for all $k$, $\theta^{( k)}|x^{( k)}| > 1$.

Well, if $\sign(x^{(k)}) = \sign(x^{(k+1)})$, then
\[
\theta^{( k+1)}|x^{( k+1)}| = \theta^{(k)}|x^{(k)}| - (\gamma^{(k)})^2
\]
and thus we can sum
\[
\theta^{(k)}|x^{(k)}| = \theta^{(0)}|x^{(0)}| - \sum_{i=1}^{k-1}(\gamma^{(i)})^2.
\]
As long as there exists a $\bar k$ where $\sum_{i=1}^{k-1}(\gamma^{(i)})^2 > 1$, then our condition is satisfied.

To find this $\bar k$, we can bound
\[
\sum_{i=1}^{k-1} (\gamma^{(i)})^2 \geq \int_1^{k-1} (\gamma^{(i)})^2 di =  \int_1^{k-1} (\frac{c}{c+i})^2 dx = \frac{c^2}{c+1}-\frac{c^2}{c+k-1}
\]
which is $\geq 1$ when
\[
k\geq \frac{3c^2-1}{c^2-c-1}.
\]
\end{proof}




\begin{lemma}
Consider the problem 
\[
\minimize{x}\quad \left\{\frac{1}{p} x^p : -1\leq x \leq 1\right\}
\]
where $p$ is even and positive. Assume that for all $\gamma^{(k)}$,
\[
\frac{\gamma^{(k+1)}}{1-\gamma^{(k+1)}} \geq \gamma^{(k)},\qquad \forall k.
\]
Then Frank-Wolfe Midpoint Method will never oscillate, for all initializations.
\end{lemma}
\begin{proof}
The midpoint method iteration scheme is:
\[
\Delta x^{(k)}_1 =  - \gamma^{(k)}(x^{(k)} + \sign(x^{(k)})), \qquad \Delta x^{(k)}_2 = - \gamma^{(k+1)}(x^{(k)}+\Delta x^{(k)}_1 + \sign(x^{(k)}+\Delta x^{(k)}_1)),
\]
\[
x^{(k+1)} = x^{(k)} + \frac{1}{2}(\Delta x^{(k)}_1 + \Delta x^{(k)}_2)
\]


First, suppose that $|x^{(k)}| < \frac{\gamma^{(k)}}{1-\gamma^{(k)}} $. This implies 
\[
\sign(x^{(k)}+\Delta x_1^{(k)}) \neq \sign(x^{(k)}).
\]
Without loss of generality, $\sign(x^{(k)}) = 1$. Then
\[
\Delta x^{(k)}_1 =  - \gamma^{(k)}(x^{(k)} +1), \qquad \Delta x^{(k)}_2 = - \gamma^{(k+1)}(x^{(k)}+\Delta x^{(k)}_1 -1),
\]
and
\begin{eqnarray*}
x^{(k+1)} &=& x^{(k)} + \frac{1}{2}(\Delta x^{(k)}_1 + \Delta x^{(k)}_2)\\
&=&x^{(k)} - \frac{\gamma^{(k)}}{2}(x^{(k)}+1) - \frac{\gamma^{(k+1)}}{2}(x^{(k)}+\Delta x^{(k)}_1 -1)\\
&=&x^{(k)} - \frac{\gamma^{(k)}}{2}(x^{(k)}+1) - \frac{\gamma^{(k+1)}}{2}(x^{(k)}-\gamma^{(k)}(x^{(k)}+1) -1)\\
&=& \left(1-\frac{\gamma^{(k)}}{2}-\frac{\gamma^{(k+1)}}{2}+\frac{\gamma^{(k+1)}\gamma^{(k)}}{2}\right)x^{(k)} -\frac{\gamma^{(k)}}{2}+\frac{\gamma^{(k)}\gamma^{(k+1)}}{2}+\frac{\gamma^{(k+1)}}{2}
\end{eqnarray*}
Since
{
\[
\left(1-\frac{\gamma^{(k)}}{2}-\frac{\gamma^{(k+1)}}{2}+\frac{\gamma^{(k+1)}\gamma^{(k)}}{2}\right)
%1- \frac{c}{2(c+k)}-\frac{c}{2(c+k+1)}+\frac{c^2}{2(c+k)(c+k+1)}\\
%&=& \frac{2(c+k)(c+k+1)}{2(c+k)(c+k+1)}- \frac{c(c+k+1)}{2(c+k)(c+k+1))}-\frac{c(c+k)}{2(c+k)(c+k+1)}\\
%&&+\frac{c^2}{2(c+k)(c+k+1)}\\
%&=&\frac{2(c+k)(c+k+1)-c(c+k+1)+c^2-c(c+k)}{2(c+k)(c+k+1)}\\
%&=&\frac{(c+2k)(c+k+1)-ck}{2(c+k)(c+k+1)}\\
=\frac{2k(c+k+1)+c(c+1)}{2(c+k)(c+k+1)}
>0
\]
}
and
\[
-\frac{\gamma^{(k)}}{2}+\frac{\gamma^{(k)}\gamma^{(k+1)}}{2}+\frac{\gamma^{(k+1)}}{2}=
%-\frac{c}{2(c+k)}+\frac{c^2}{2(c+k)(c+k+1)}+\frac{c}{2(c+k+1)}\\
%&=&\frac{c^2+c(c+k)-c(c+k+1)}{2(c+k)(c+k+1)}\\
\frac{c(c-1)}{2(c+k)(c+k+1)}
\overset{c\geq1}{>}0
\]
we have that $\sign(x^{(k+1)})= 1$ if $\sign(x^{(k)}) =1$
Next,, suppose that $|x^{(k)}| > \frac{\gamma^{(k)}}{1-\gamma^{(k)}} $. This implies 
\[
\sign(x^{(k)}+\Delta x_1^{(k)}) = \sign(x^{(k)}).
\]
Without loss of generality, $\sign(x^{(k)}) = 1$. Then
\[
\Delta x^{(k)}_1 =  - \gamma^{(k)}(x^{(k)} +1), \qquad \Delta x^{(k)}_2 = - \gamma^{(k+1)}(x^{(k)}+\Delta x^{(k)}_1 +1),
\]
and
\begin{eqnarray*}
x^{(k+1)} &=& x^{(k)} + \frac{1}{2}(\Delta x^{(k)}_1 + \Delta x^{(k)}_2)\\
&=&x^{(k)} - \frac{\gamma^{(k)}}{2}(x^{(k)}+1) - \frac{\gamma^{(k+1)}}{2}(x^{(k)}+\Delta x^{(k)}_1 +1)\\
&=&x^{(k)} - \frac{\gamma^{(k)}}{2}(x^{(k)}+1) - \frac{\gamma^{(k+1)}}{2}(x^{(k)}-\gamma^{(k)}(x^{(k)}+1) +1)\\
&=&\left(1-\frac{\gamma^{(k)}}{2}-\frac{\gamma^{(k+1)}}{2}+\frac{\gamma^{(k+1)}\gamma^{(k)}}{2}\right)x^{(k)} -\frac{\gamma^{(k)}}{2}+\frac{\gamma^{(k)}\gamma^{(k+1)}}{2}-\frac{\gamma^{(k+1)}}{2}\\
&> & \left(1-\frac{\gamma^{(k)}}{2}-\frac{\gamma^{(k+1)}}{2}+\frac{\gamma^{(k+1)}\gamma^{(k)}}{2}\right)\frac{\gamma^{(k)}}{1-\gamma^{(k)}} -\frac{\gamma^{(k)}}{2}+\frac{\gamma^{(k)}\gamma^{(k+1)}}{2}-\frac{\gamma^{(k+1)}}{2}\\
&=&  \left(1-\frac{\gamma^{(k)}}{2}-(1-\gamma^{(k)})\frac{\gamma^{(k+1)}}{2} \right)\frac{\gamma^{(k)}}{1-\gamma^{(k)}} -\frac{\gamma^{(k)}}{2}+\frac{\gamma^{(k+1)}}{2}(\gamma^{(k)}-1)\\
&=&  (1-\frac{\gamma^{(k)}}{2})\frac{\gamma^{(k)}}{1-\gamma^{(k)}} - \frac{\gamma^{(k+1)}\gamma^{(k)}}{2} -\frac{\gamma^{(k)}}{2}+\frac{\gamma^{(k+1)}}{2}(\gamma^{(k)}-1)\\
&=&  (1-\gamma^{(k)}+\frac{\gamma^{(k)}}{2})\frac{\gamma^{(k)}}{1-\gamma^{(k)}}  -\frac{\gamma^{(k)}}{2}
-\frac{\gamma^{(k+1)}}{2}\\
&=&  \gamma^{(k)} + (\frac{\gamma^{(k)}}{2})\frac{\gamma^{(k)}}{1-\gamma^{(k)}}  -\frac{\gamma^{(k)}}{2}
-\frac{\gamma^{(k+1)}}{2}\\
&\geq& 0
\end{eqnarray*}

\end{proof}

\newpage
\begin{corollary}
Consider the problem
\begin{equation}
\minimize{x}\quad \{\frac{1}{p}\|x\|_2^p:\|x\|_\infty \leq \alpha\}
\label{eq:shifted-infnorm-example}
\end{equation}
where $p$ is even. Then the vanilla Frank-Wolfe method will always oscillate after some finite iterate, and the midpoint method will never oscillate. 
\end{corollary}

\begin{proof}
 


\[
\nabla f(x) = \|x\|_2^{p-2} x
\]

\[
s = \bmat \sign(x_1)\\\sign(x_2)\\\vdots\\\sign(x_n)\emat
\]

The iteration scheme is exactly the same as if we independently update $x_i$ at each iteration.
\end{proof}


\begin{theorem}
Consider the problem
\[
\minimize{x} \quad \{\frac{1}{p}\|x\|_2^p : \|x\|_1\leq \alpha\}
\]
Then, for Frank Wolfe, for each $i = 1,...,n$, either
$|x_i^*| > 0$  or $x_i^{(k)}$ must oscillate an infinite number of times.

However, midpoint method will not oscillate.

\end{theorem}


\begin{theorem}
Consider the problem
\[
\minimize{x} \quad \{\frac{1}{p}|x-b| : |x|\leq \alpha\}
\] 
\end{theorem}




\red{todo: extension to extragradient method, should oscillate.}

\red{todo: extend to 1-norm set}


        \red{Maybe need a negative result for rk methods}
        
        
\gray{ Runge Kutta discretizes the Frank Wolfe flow as:
For some choice of $A\in \R^{q\times q}$, $b\in \R^q$, and $c\in \R^q$, a $q$-stage discretization methods can be written as (at step $k$, for $i = 1,...,q$)
\begin{equation}
  \Delta {\bx}_{i-1} = \gamma_{k+c_{i-1}}(\bs_{i-1}-(\bx^{(k)}+\bar{\bx}_{i-1})),\quad \bar{\bx}_i = \sum_{j < i } A_{ij} \Delta{\bx}_j, \quad 
\bs_i = \lmo_\mD(\bx^{(k)}+\bar{\bx}_i),
\label{eq:general_discrete}
  \end{equation}
where $\bar{\bx}_0 = 0$ and the next step $\bx^{(k+1)} = \bx^{(k)} + \sum_{i=1}^q b_i\Delta{\bx}_i$.
When we use Runge Kutta meghods, the convergence rate is always $O(\frac{1}{t})$.
\begin{proof}

\end{proof}
}
\fi
